First Steps Toward a Method for Estimating Cosmological Parameters using Strong Lensing, X-ray and Dynamics Total Mass Estimates

In this thesis we want to introduce the first steps towards realising a new method to investigate the cosmological parameters and conduct a detailed analysis of the galaxy cluster MACS J0416. Toward this end, we use the current model from Grillo et al. (2015) as a template and the publicly available lensing code Lenstool. This code has previously been used by Jauzac et al. (2014), Richard et al. (2014), Jauzac et al. (2015) and Caminha et al. (2016) to model MACS J0416 (Grillo et al. (2015) used GLEE). We created $10$ different models to cover a reasonable set of different approaches. In addition to the replication of the Grillo et al. (2015) models, with two cluster scale halos and 175 circular cluster member mass-density profiles, we created models using elliptical mass-density profiles for the cluster members and models where we optimize the cluster member scaling relation slopes. In order to investigate the viability of using the projected total mass estimate from different cosmological models to estimate the cosmological parameter values, we created 49 models each representing a different set of cosmological parameters.

==> chapterCP3.tex <==
%auto-ignore
\usepackage{soul}

%%%%%%%%%%%%					%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  Kapitel layout 	%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%					%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter 
\newlength\dlf@normtxtw 
\setlength\dlf@normtxtw{\textwidth} 
\def\myhelvetfont{\def\sfdefault{mdput}} 
\newsavebox{\feline@chapter} 

\newcommand\feline@chapter@marker[1][4cm]{%
	\sbox\feline@chapter{% 
		\resizebox*{!}{#1}{\fboxsep=1pt%
			\colorbox{moerkeroed}{\color{white}\bfseries\sffamily\thechapter}% 
		}}%
	\rotatebox{90}{% 
		\resizebox{%
			\heightof{\usebox{\feline@chapter}}+\depthof{\usebox{\feline@chapter}}}% 
		{!}{\scshape\so\@chapapp}}\quad%
	\raisebox{\depthof{\usebox{\feline@chapter}}}{\usebox{\feline@chapter}}%
} 
		
\newcommand\feline@chm[1][4cm]{%
	\sbox\feline@chapter{\feline@chapter@marker[#1]}% 
	\makebox[0pt][l]{% aka \rlap
	\makebox[0cm][r]{\usebox\feline@chapter}%
	}} 

\makechapterstyle{kap}{
	\renewcommand\chapnamefont{\normalfont\Large\scshape\raggedleft\so} 
	\renewcommand\chaptitlefont{\normalfont\Huge\bfseries\scshape\color{moerkeroed}} 
	\renewcommand\chapternamenum{} \renewcommand\printchaptername{} 
	\renewcommand\printchapternum{\hfill\feline@chm[2.5cm]\par} 
	\renewcommand\afterchapternum{\par\vskip\midchapskip} 
	\renewcommand\printchaptertitle[1]{\chaptitlefont\raggedleft ##1\par}
}


%%%%%%%%%%%%					%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  Kapitel layout 2	%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%					%%%%%%%%%%%%%%%%%%%%%%%%

%\makeatletter 
%\newlength\dlf@normtxtw 
%\setlength\dlf@normtxtw{\textwidth} 
%\def\myhelvetfont{\def\sfdefault{mdput}} 
%\newsavebox{\feline@chapter} 
%
%\newcommand\feline@chapter@marker[1][4cm]{%
%	\sbox\feline@chapter{% 
%		\resizebox*{!}{#1}{\fboxsep=1pt%
%			\colorbox{moerkeroed}{\color{white}\bfseries\sffamily\thechapter}% 
%		}}%
%	\rotatebox{90}{% 
%		\resizebox{%
%			\heightof{\usebox{\feline@chapter}}+\depthof{\usebox{\feline@chapter}}}% 
%		{!}{\scshape\so\@chapapp}}\quad%
%	\raisebox{\depthof{\usebox{\feline@chapter}}}{\usebox{\feline@chapter}}%
%} 
%		
%\newcommand\feline@chm[1][4cm]{%
%	\sbox\feline@chapter{\feline@chapter@marker[#1]}% 
%	\makebox[0pt][l]{% aka \rlap
%	\makebox[2.5cm][r]{\usebox\feline@chapter}%
%	}
%	} 
%
%\makechapterstyle{kap2}{
%	\renewcommand\chapnamefont{\normalfont\Large\scshape\raggedleft\so} 
%	\renewcommand\chaptitlefont{\normalfont\Huge\bfseries\scshape\color{moerkeroed}} 
%	\renewcommand\chapternamenum{} 
%	\renewcommand\printchaptername{} 
%	\renewcommand\printchapternum{\feline@chm[2.5cm]} 
%	\renewcommand\afterchapternum{\hfill} 
%	\renewcommand\printchaptertitle[1]{\chaptitlefont\raggedleft ##1\par}
%}
%

\makeatother 
\chapterstyle{kap}

\newcommand{\ruledsec}[1]{% 
\Large\bfseries\slshape \raggedleft \textcolor{moerkeroed}{#1} \vspace{-3mm} \rule{\textwidth}{0.2pt}\vspace{-8mm}}
\newcommand{\redsec}[1]{% 
\noindent\Large\bfseries \textcolor{moerkeroed}{#1}}
\setsecheadstyle{\redsec}%\Large \bfseries\slshape \raggedleft}
\newcommand{\subsec}[1]{%
\large \bfseries\slshape\color{moerkeroed} #1 \vspace{-0mm}}
\setsubsecheadstyle{\subsec}%\large \bfseries\color{moerkeroed}}
\newcommand{\subsubsec}[1]{%
\fontsize{12.5pt}{1em} \bfseries\color{moerkeroed} #1 \vspace{-2mm}}
\setsubsubsecheadstyle{\subsubsec}%\large \bfseries\color{moerkeroed}}



